Stability of Dusty Rings in Protoplanetary Discs

Dust rings in protoplanetary discs are often observed in thermal dust emission and could be favourable environments for planet formation. While dust rings readily form in gas pressure maxima, their long-term stability is key to both their observability and potential to assist in planet formation. We investigate the stability of the dust ring generated by interactions of a protoplanetary disc with a Neptune sized planet and consider its possible long term evolution using the FARGO3D Multifluid code. We look at the onset of the Rossby Wave Instability (RWI) and compare how the addition of dust in a disc can alter the stability of the gas phase. We find that with the addition of dust, the rings generated by planet disc interactions are more prone to RWI and can cause the gas phase to become unstable. The instability is shown to occur more easily for higher Stokes number dust, as it accumulates into a more narrow ring which triggers the RWI, while the initial dust fraction plays a more minor role in the stability properties. We show that the dusty RWI generates vortices that collect dust in their cores, which could be sites for further planetesimal formation. We conclude that the addition of dust can cause a ring in a protoplanetary disc to become more prone to instability leading to a different long term evolution compared to gas only simulations of the RWI.

==> notes.tex <==


\begin{figure}
\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Plots/02st_keyavg.png[draft]}
\end{subfigure}
\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Plots/02st_key.png[draft]}
\end{subfigure}
\caption{key t=100}
\label{fig:t100key}
\end{figure}




DRAG CUTOFF

\begin{figure}
\includegraphics[width=\linewidth]{Plots/cut_mix_total.png[draft]}
\caption{$Cut mix total 70,80,90$} 
\label{fig:cutmixtotal}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{Plots/cut_gas_t90.png[draft]}
\caption{$Cut gas t 90$} 
\label{fig:cutgas}
\end{figure}


LONG

\begin{figure}
\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Plots/02st_densplot_t110a.png[draft]}
\end{subfigure}
\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Plots/02st_densplot_t110.png[draft]}
\end{subfigure}
\caption{t = 110}
\label{fig:t110dens}
\end{figure}

\begin{figure}
\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Plots/02st_densplot_t200a.png[draft]}
\end{subfigure}
\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Plots/02st_densplot_t200.png[draft]}
\end{subfigure}
\caption{t = 200}
\label{fig:t200dens}
\end{figure}


\newpage
\section{Notes}

\begin{itemize}
  \item RWI triggered by axisymmetric bump, key function (analytically, \citealt{lovelace99}; \citealt{li00a} and numerically, \citealt{li00b}; \citealt{varniere06})
  \item Gives rise to high pressure anticyclonic vortices that trap dust in the center through drag
  \item Survival of vortices on a sufficient timescale may be a problem, due to destruction (elliptical instability, \citealt{lesur09}) or migration (\citealt{paardekooper10})
  \item\cite{meheut12a} shows in 3D discs that Rossby vortices can survive for hundreds of years without migrating, then are isolated (\citealt{godon00}; \citealt{lesur09}) and prone to elliptical instability and viscous decay if not sustained.
  \item Project to investigate stability of exterior dusty rings produced by Neptune sized planet
  \item RWI triggers vortices at location of ring and density waves are emitted from the region of density extremum
  \item How stable are the dusty rings caused by planets?
\end{itemize}

\cite{huang20} - 

\begin{itemize}
    \item two fluid simulations of dusty ring formed by gas over-density in dead-zone
    \item dead-zone introduces transition between low and high viscosity which leads to over-density
    \item width of the transition zone changed from 2,3,4H , dust fraction of 0.05
    \item 2H width shows formation of many small vortices at outer edge of dusty ring, destruction of vortices by strong dust feedback (\citealt{fu14b}) and new phase of instabilities generating vortices again
    \item 3H, 4H - no dust clumps
    \item meso-scale instability 
\end{itemize}

\cite{lee22} -

\begin{itemize}
    \item 2D shearing box simulation
    \item Gaussian pressure perturbation via forcing (akin to zonal winds, ice condensations) or tidal interaction with planet
    \item GIZMO Lagrangian mesh-less finate mass method
    \item Super-particle which represents ensemble of dust grains
    \item Dust collects away from centre of pressure bump, larger $t_s$ collects into thinner rings
    \item Under planet forcing, dust rings start narrow then widen with time with drift diffusion steady state
\end{itemize}

\cite{pierens21}

\begin{itemize}
    \item secular gravitational instability to generate ringed structures
    \item this may lead to planetesimal formation during non-linear phase of instability
    \item 2D simulations with self gravity using GENESIS with FARGO algorithm
    \item L1 model: higher Stokes, no dust diffusion, particle velocity dispersion
    \item linear evolution of dust rings lead into non-linear evolution with ring fragmentation into dusty clumps
    \item SGI creates rings, rings become thinner as gravitational collapse proceeds, then leads to RWI
    \item formation of dust clumps result from RWI which is expected at bumps in the potential vorticity
    \item Rossby Number plot (see their Eq. 15)
    \item L2 model: lower Stokes, dust diffusion constant, no particle velocity dispersion
    \item mode 1 spiral wave develops
\end{itemize}

\begin{itemize}
    \item Rossby Wave Instability 
    \item Streaming Instability - sub-Keplerian gas causes headwind on dust, dust migrates in, clumps together, backreaction drags gas, reducing local headwind. Isolated particles join clump, further reducing headwind, increasing clump size. Care for high dust to gas ratios.
    \item Elliptical Instability - Lesur \& Papaloizou 2009, instability found in elliptical vortex cores, resonance between turnover time and local epcyclic oscillation period, core can be stable at certain aspect ratio however boundary is unstable. Found at small scales and can be weak.
\end{itemize}


%Initially, we present the key function plots for a gas only disc in Fig. \ref{fig:gas5e-7}. We see that in this plot with a kinematic viscosity of $\nu = 5\times 10^{-7}$ which is between the second and third plot of Fig. \ref{fig:ngasonlycombo}, whereby one gap edge triggered the RWI and one did not, the gas only disc does not generate vortices at the disc gap edge that would disrupt the ring structure exterior or interior to the planet. Later on there may be enough of a buildup to trigger the RWI however at this stage the conditions for the instability to trigger has not been met even though peaks are shown in the azimuthally averaged key function plot (top of Fig. \ref{fig:gas5e-7}) at the location of the gap edges. 

%The 2D key function plot (bottom of Fig. \ref{fig:gas5e-7}) shows smooth gap edges unlike the lower kinematic viscosity plots from the previous subsection. As the control case we intended to show how the addition of dust could affect the gas phase, whether it would trigger the RWI earlier or suppress it as the dust interacts with the gas. Additionally we cautiously evaluate the radial profile of the "mixed" key function (eq. \ref{keyfuncmix}) and if it has the same indications as the radial profile of the key function (eq. \ref{keyfuncgas}).
